Period functions for vector-valued Maass cusp forms of real weight, with an application to Jacobi Maass cusp forms

For vector-valued Maass cusp forms for~$SL_2(\mathbb{Z})$ with real weight~$k\in\mathbb{R}$ and spectral parameter $s\in\mathbb{C}$, $\mathrm{Re} s\in (0,1)$, $s\not\equiv \pm k/2$ mod $1$, we propose a notion of vector-valued period functions, and we establish a linear isomorphism between the spaces of Maass cusp forms and period functions by means of a cohomological approach. The period functions are a generalization of those for the classical Maass cusp forms, being solutions of a finite-term functional equation or, equivalently, eigenfunctions with eigenvalue $1$ of a transfer operator deduced from the geodesic flow on the modular surface. We apply this result to deduce a notion of period functions and related linear isomorphism for Jacobi Maass forms of weight $k+1/2$ for the semi-direct product of $SL_2(\mathbb{Z})$ with the integer points $Hei(\mathbb{Z})$ of the Heisenberg group.

==> rwt7-not.tex <==
% mainfile: rwt7.tex



% general definitions

\usepackage{amssymb,amsmath,amsthm}


\usepackage[all]{xy}
\usepackage{graphicx}

\usepackage{enumitem}

\makeatletter
%\@ifundefined{iflabels}{}{%
%\iflabels
%\usepackage[notcite,notref]{showkeys}
%\fi}

\@ifundefined{iftxfonts}{\usepackage[varg]{txfonts}}{%
\iftxfonts
\usepackage[varg]{txfonts}
% gives nicer result when printing
\fi}


\@ifundefined{ifindex}{\let\ifindex=\iffalse}{}

\makeatother


% \grf{width in cm}{filename }
% to be put in center environment
\newcommand\grf[2]{
\includegraphics[width=#1cm]{pict/#2.pdf}}


%file name at bottom of pages
\iffalse
\makeatletter \@ifundefined{version}{\def\version{}}{}
\@ifundefined{flnm}{}{%
% file name on bottom of page
\def\@oddfoot{\rm{\footnotesize{File name
\tt\flnm\version.tex}\quad\today\hfil\thepage}}
\let\@evenfoot\@oddfoot \addtolength{\textheight}{-.4cm}
\addtolength{\footskip}{.4cm} }
\makeatother
\fi


%%%%%%%%%% hyperref %%%%%%%%%%%%%%%%%%%%%%5

\let\ifhyperref=\iftrue
\makeatletter \@ifundefined{ifhyperref}{\let\ifhyperref=\iffalse}{}
\makeatother


\ifhyperref
% experiment whether hyperlinks can be made to work
  \usepackage[colorlinks,breaklinks,pdfpagelabels,hypertexnames=false]{hyperref}
\else
  \newcommand\texorpdfstring[2]{#1}
\fi

\let\synctex=1

%%% equations, theorem, ...
\def\be#1\ee{\begin{equation}#1\end{equation}}
\def\bad#1\ead{\be\begin{aligned}#1\end{aligned}\ee}
\def\badl#1#2\eadl{\be\label{#1}\begin{aligned}#2\end{aligned}\ee}
\let\ovln\=
\renewcommand\={\,=\,}


\newtheorem{thm}{Theorem}[section]
\newtheorem{prop}[thm]{Proposition}
\newtheorem{cor}[thm]{Corollary}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{guess}[thm]{Guess}
\newtheorem{mainthm}{Theorem}
\renewcommand{\themainthm}{\Alph{mainthm}}

\theoremstyle{definition}
\newtheorem{defn}[thm]{Definition}
\newtheorem{remark}[thm]{Remark}
\newtheorem{quest}[thm]{Question}

\newcommand\rmrk[1]{\medskip\par\noindent\emph{#1. }}

\theoremstyle{remark}
\newtheorem*{ack}{Acknowledgement}


%%%% color %%%%


\usepackage{color}
\definecolor{blue}{rgb}{0,0,1}
\definecolor{red}{rgb}{1,0,0}
\definecolor{green}{rgb}{0,.6,.2}
\definecolor{purple}{rgb}{1,0,1}
\definecolor{brown}{rgb}{.59,.29,0}

\long\def\red#1\endred{{\color{red}#1}}
\long\def\blue#1\endblue{{\color{blue}#1}}
\long\def\purple#1\endpurple{{\color{purple} #1}}
\long\def\green#1\endgreen{{\color{green}#1}}
\long\def\brown#1\endbrown{{\color{brown}#1}}


%%%%%%%%%%%%%%% Greek letters
\newcommand\al{\alpha}
\newcommand\Bt{{\mathsf{B}}}
\newcommand\bt{\beta}
\newcommand\Gm{\Gamma}
\newcommand\gm{\gamma}
\newcommand\Dt{\Delta}
\newcommand\dt{\delta}
\newcommand\e{\varepsilon}
\newcommand\z{{\zeta}}
\newcommand\Eta{{\mathsf{H}}}
\newcommand\Th{\Theta}
\renewcommand\th{\vartheta}
\renewcommand\k{\kappa}
\newcommand\Ld{\Lambda}
\newcommand\ld{\lambda}
\newcommand\x{\xi}
\renewcommand\r{\rho}
\newcommand\Sg{\Sigma}
\newcommand\s{\sigma}
\newcommand\Ups{\Upsilon}
\newcommand\ups{\upsilon}
\newcommand\Ph{\Phi}
\newcommand\ph{\varphi}
\newcommand\ch{\chi}
\newcommand\Ps{\Psi}
\newcommand\ps{\psi}
\newcommand\Om{\Omega}
\newcommand\om{\omega}


%%%%%%%%%%%%%%%% general notations
\newcommand\re{{\mathrm{Re}\,}}
\newcommand\im{{\mathrm{Im}\,}}
\newcommand\SL{{\mathrm{SL}}}
\newcommand\PSL{{\mathrm{PSL}}}
\newcommand\GL{{\mathrm{GL}}}
\newcommand\PGL{{\mathrm{PGL}}}
\newcommand\SU{{\mathrm{SU}}}
\newcommand\SO{{\mathrm{SO}}}
\newcommand\U{{\mathrm{U}}}
\newcommand\Sp{{\mathrm{Sp}}}
\newcommand\Mp{\mathrm{Mp}}



%%%%%%%%%%%%% blackboard boldface
\newcommand\CC{\mathbb{C}}
\newcommand\HH{\mathbb{H}}
\newcommand\NN{\mathbb{N}}
\newcommand\QQ{\mathbb{Q}}
\newcommand\RR{\mathbb{R}}
\newcommand\ZZ{\mathbb{Z}}

%%%%%%%%%%%% matrices
%\makeatletter
%in amsmath  \atop  is redefined, \@@atop is left
%\newcommand\rmatc[4]{\left( {#1\@@atop #3}{#2\@@atop #4}\right)}
%\newcommand\rmatr[4]{\left( {\hfill #1\@@atop\hfill #3}{\hfill
%#2\@@atop\hfill #4}\right)}
%\newcommand\matc[4]{\left[ {#1\@@atop #3}{#2\@@atop #4}\right]}
%\newcommand\matr[4]{\left[ {\hfill #1\@@atop\hfill #3}{\hfill
%#2\@@atop\hfill #4}\right]}
%\makeatother
\newcommand\rmatc[4]{\begin{pmatrix}#1&#2\\#3&#4\end{pmatrix}}
\let\rmatr=\rmatc
\newcommand\matc[4]{\begin{bmatrix}#1&#2\\#3&#4\end{bmatrix}}
\let\matr=\matc

\let\setminus\smallsetminus
\newcommand\dis{\stackrel{\hbox{.}}=}
\newcommand\ddis{\,\dis\,}


%%%%%%%%% other notations %%%%%%%%%%%%%%

\newcommand\lijn{\bigskip\par\hrule\bigskip\par}
\newcommand\hp{{\mathfrak H}}
\let\uhp\hp
\newcommand\lhp{\hp^-}
\newcommand\hypg[2]{{}_{#1}F_{\!#2}}

\newcommand\divides{\,\mid\,}
\newcommand\dividesnot{\,\not\mid\,}

\newcommand\summ[2]{\mathop{\sum{\!\raisebox{1.2ex}{{$#1$}}}}_{\!\!#2}}


\newcommand\sign{\operatorname{Sign}}
\newcommand\supp{\operatorname{Supp}}
\newcommand\Gf{\Gamma}
\newcommand\oh{{\mathrm{O}}}
\newcommand\proj[1]{\mathbb{P}^1_{\!#1}}
\newcommand\projj[2]{\mathbb{P}^{#1}_{\!#2}}

\newcommand\intitle[1]{\texorpdfstring{$#1$}{}}

%\newcommand\res{{\mathop{\mathrm{Res}}}}

\newcommand\rest{{\mathrm{res}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\renewcommand\theequation{\arabic{section}.\arabic{equation}}
\numberwithin{equation}{section}

\newcommand\tm{\tilde T}
\newcommand\sm{\tilde S}

\newcommand\A{{\mathcal A}}

\newcommand\V[2]{\mathcal{V}^{#1}_{\!#2}}
\newcommand\tV[2]{\tilde{\mathcal{V}}^{#1}_{\!#2}}
\newcommand\lm{\mathrm{lm}}
\newcommand\exc{\mathrm{exc}}

\newcommand\W[2]{\mathcal{W}^{#1}_{\!#2}}

\newcommand\G[2]{\mathcal{G}^{#1}_{\!#2}}
\newcommand\N[2]{\mathcal{G}^{#1}_{\!#2}}

\newcommand\km{{\mathrm k}}
\newcommand\am{{\mathrm a}}
\newcommand\nm{{\mathrm n}}
\newcommand\hm{{\mathrm h}}

\newcommand\hei{{\mathsf{Hei}}}

\newcommand\B{{\mathcal B}}

\renewcommand\H{{\mathbf H}}
\newcommand\XX{{\mathbf X}} 
\newcommand\WW{{\mathbf W}}
\newcommand\EE{{\mathbf E}}
\newcommand\Q{{\mathbf Q}}
\newcommand\glie{{\mathfrak g}}
\newcommand\lieJ{{\mathfrak g}^J}
\newcommand\prs{\mathrm{ps}}
\newcommand\E{{\mathcal E}}
\newcommand\coh{{\mathbf r}}
\newcommand\pb{\mathrm{par}}
\newcommand\FE{\mathsf{FE}}
\newcommand\tFE{{}^{w}\FE}
\newcommand\pr{{\mathrm{pr}}}
\newcommand\ppm{{\mathrm{p}}}
\newcommand\YY{{\mathbf{Y}}}
\newcommand\DD{{\mathbf{D}}}
\newcommand\lnm{{\mathrm{lm}}}
\newcommand\Cas{\mathcal{C}}


\renewcommand\atop[2]{\mathchoice{\genfrac{}{}{0pt}{0}{#1}{#2}}%
  {\genfrac{}{}{0pt}{1}{#1}{#2}}%
  {\genfrac{}{}{0pt}{2}{#1}{#2}}%
  {\genfrac{}{}{0pt}{3}{#1}{#2}}%
  }
  
\newcommand\cu{{\mathcal C}}

\newcommand\tro{{\mathcal{L}}}
\newcommand\trof[1]{{\mathcal{L}_{#1}^{\mathrm{fast}}}}
\newcommand\av[1]{{\mathrm{A\!v}^{\!#1}}}
\newcommand\fd{\mathfrak{F}}
\newcommand\Fa{{\mathsf{Ft}}}

\ifhyperref
\newcommand\tocrgl[2]{
\addtocontents{toc}{\string\contentsline{subsection}
{\blue  #1, #2\endblue} {\thepage}
{}}}
\else
\newcommand\tocrgl[2]{\addtocontents{toc}%
{\string\contentsline{subsection}%
{\blue  #1, #2 \endblue}
{\thepage}%
{}}}
\fi

%\newcommand\change[2]{\marginpar{\red change \endred}\footnote{Change #1:  #2}%
% \tocrgl{Change}{#1}}
 
%\newcommand\rem[2]{\marginpar{\red remark \endred}\footnote{Remark #1:  #2}%
% \tocrgl{Remark}{#1}}
 
 
%\newcommand\qstn[2]{\marginpar{\red question \endred}\footnote{Question #1:  #2}%
% \tocrgl{Question}{#1}}
 
 \newcommand\hg[1]{{}^{#1\!}}

\renewcommand\pr{\mathrm{pr}\,}
\newcommand\tG{\tilde G}
\newcommand\tGm{\tilde \Gm}
\newcommand\tppm{\tilde{\mathrm{p}}}
\newcommand\tkm{\tilde{\mathrm{k}}}
\newcommand\tam{\tilde{\mathrm{a}}}
\newcommand\tg{\tilde g}
\newcommand\tZ{\tilde Z}
\newcommand\tK{\tilde K}
\newcommand\tA{\tilde A}
\newcommand\gj{{\mathbf{g}}}


\newcommand\pf{\mathrm{pf}}
\newcommand\Fbg[1]{{\mathcal{F}_{\!#1}}}

\newcommand{\tth}{\vec\th}


%%% macros for index
\usepackage{multicol}
\makeatletter
\@ifundefined{ifindexindication}{\let\ifindexindication=\iffalse}{}
\ifindexindication
 \newcommand\indexindication[2]
 {\raisebox{1.6ex}{\makebox[0cm][#2]{\tiny #1}}}
 \newcommand\il[2]{\label{i-#1}\indexindication{#2}{l}}
 \newcommand\ir[2]{\indexindication{$#2$}{r}}
\else
 \newcommand\il[2]{\label{i-#1}}
 \newcommand\ir[2]{}
\fi
\makeatother
% second argument of \il and \ir is not used in composing the index,
% since that is done by hand.
% in \ifindexindication is true then the second argument of \il
% need to be in text mode (so use $ around formulas)
% the second argument of \ir needs to be in math mode


